Learning for Counterfactual Fairness from Observational Data

Fairness-aware machine learning has attracted a surge of attention in many domains, such as online advertising, personalized recommendation, and social media analysis in web applications. Fairness-aware machine learning aims to eliminate biases of learning models against certain subgroups described by certain protected (sensitive) attributes such as race, gender, and age. Among many existing fairness notions, counterfactual fairness is a popular notion defined from a causal perspective. It measures the fairness of a predictor by comparing the prediction of each individual in the original world and that in the counterfactual worlds in which the value of the sensitive attribute is modified. A prerequisite for existing methods to achieve counterfactual fairness is the prior human knowledge of the causal model for the data. However, in real-world scenarios, the underlying causal model is often unknown, and acquiring such human knowledge could be very difficult. In these scenarios, it is risky to directly trust the causal models obtained from information sources with unknown reliability and even causal discovery methods, as incorrect causal models can consequently bring biases to the predictor and lead to unfair predictions. In this work, we address the problem of counterfactually fair prediction from observational data without given causal models by proposing a novel framework CLAIRE. Specifically, under certain general assumptions, CLAIRE effectively mitigates the biases from the sensitive attribute with a representation learning framework based on counterfactual data augmentation and an invariant penalty. Experiments conducted on both synthetic and real-world datasets validate the superiority of CLAIRE in both counterfactual fairness and prediction performance.

==> deriv.tex <==
\section{Derivation}

\begin{figure}[tbh!]
    \vspace*{-0.3cm}
    \begin{minipage}{0.49\textwidth}
        \centering
        % \resizebox{\textwidth}{!}{
      \tiny \begin{tikzpicture}
\centering

    \node[state] (s) at (0,1) {$S$};
    \node[state] (x1) at (0,0) {${X}_1$};

    \node[state] (y) at (2,0) {$Y$};
    \node[state] (x2) at (4,0) {${X}_2$};
        \node[state] (u) at (-2,0) {$U$}; 
          \node[state] (x3) at (2,1) {${X}_3$};

    % Directed edge
    % \path [bidirected,black,line width=1.5] (e) edge (xc);
    \path  (s) edge (x1);
        \path  (u) edge (x1);
              \path  (x1) edge (y);      
              \path  (x3) edge (y);     
              \path  (y) edge (x2);
                     \path  (s) edge (x2);
                            \path  (s) edge (y);
    % \path [black,line width=1.5] (xc) edge (y);

\end{tikzpicture}
        % }
        % \vspace{-0.1cm}
\caption{
% The causal relationships among the causal features $X^c$, the spurious features $X^s$, the domain label $E$ and the class label $Y$ in OOD prediction.
    %
    % The influence of $E$ on $Y$ is mediated by the causal features ${X}^c$.
    %
    The causal graph showing the motivation of the proposed framework
    %
    % The thick edges show strong $\Lambda$ spuriousness.
    }
    \label{fig:causal_graph_example}
    \end{minipage}
    \end{figure}
    
    \begin{equation}
        \begin{split}
            S &= \mathcal{N}(0,\sigma_S^2)\\
                        U &= \mathcal{N}(0,\sigma_U^2)\\
                    X_1 &= S + U + \mathcal{N}(0,\sigma_1^2)\\
              Y &= X_1 + X_3 + \mathcal{N}(0,\sigma_Y^2)\\
                            X_2 &= Y + \mathcal{N}(0,\sigma_2^2)\\X_3 &= \mathcal{N}(0,\sigma_3^2)
        \end{split}
        \label{eq:sem}
    \end{equation}
    
    Given the causal graph in Fig.~\ref{fig:causal_graph_example} and the structural equations in Eq.~\ref{eq:sem}. We assume that all the noise are i.i.d. samples from the corresponding Gaussian distributions.
    %
    We further assume that $\sigma_1$, $\sigma_Y$ and $\sigma_2$ depend on the value of $S$.
    %
    We consider different combinations of features, the corresponding regression models $\hat{P}(Y|X_3)$, $\hat{P}(Y|X_3,X_1)$, $\hat{P}(Y|X_3,X_1,X_2)$, and $\hat{P}(Y|X_3,U)$ to check their prediction errors and unfairness.
    %
    
    First, we consider, $\hat{P}(Y|X_3)$, where the features are the causal features which are not descendants of the sensitive attribute.
    %
    We will end up with $\hat{Y} = X_3$.
    %
    This model is invariant as the coefficient is constant.
    %
    But we find its residual $\hat{Y}-Y = \mathcal{N}(0,\sigma_Y^2+\sigma_1^2+\sigma_S^2+\sigma_U^2)$ has large variance.
    %
    This model is completely fair, that means $\hat{Y}_{S\leftarrow s} - \hat{Y}_{S\leftarrow s'} = 0,s \not = s'$.
    %
    
    Second, we consider $\hat{P}(Y|X_1,X_3)$. With OLS estimator, we will have $\hat{Y} = X_1+X_3$.
    %
    In this case, the model's unfairness is $\hat{Y}_{S\leftarrow s} - \hat{Y}_{S\leftarrow s'} \sim \mathcal{N}(0,\sigma_s^2+\sigma_{s'}^2)$.
    %
    The residual is $\hat{Y}-Y = \mathcal{N}(0,\sigma_Y^2)$.
    The model is also invariant.
    %
    
    Third, for model $\hat{P}(Y|X_1,X_2,X_3)$. We will have $\hat{Y} = \frac{\sigma_2^2}{\sigma_2^2+\sigma_Y^2}X_1+\frac{\sigma_Y^2}{\sigma_2^2+\sigma_Y^2}X_2+\frac{\sigma_2^2}{\sigma_2^2+\sigma_Y^2}X_3$.
    %
    We can see this model is not invariant as its coefficients rely on variables that depend on the value of $S$.
    %
        Its residual is $\hat{Y}-Y \sim \mathcal{N}(0,2\frac{\sigma_2^4 \sigma_Y^2}{(\sigma_2^2+\sigma_Y^2)^2}).$
    %
    This implies that when $S$ takes an arbitrary value in the unseen test set, the worst case prediction error can be extremely large.
    %
    This model's unfairness is $\hat{Y}_{S\leftarrow s} - \hat{Y}_{S\leftarrow s'} \sim \mathcal{N}(0,\frac{(\sigma_2^4+\sigma_Y^4)(\sigma_{s}^2+\sigma_{s'}^2)}{(\sigma_2^2+\sigma_Y^2)^2})$.
    %

    
   Finally, if we consider the oracle model $\hat{P}(Y|X_3,U)$, we will obtain the linear regression model $\hat{Y} = X_3+U$ through the OLS estimator.
   %
   We find this model is invariant as the coefficients are constant. It is also fair as $\hat{Y}_{S\leftarrow s} - \hat{Y}_{S\leftarrow s'} = 0$.
   %
   Its residual is $\hat{Y}-Y \sim \mathcal{N}(\sigma_Y^2+\sigma_1^2+\sigma_S^2)$.
   %
   Based on such results, we can conclude the oracle model is better than all models mentioned above.
   %
   However, as $U$ is a hidden variable, this model cannot be directly learned from observed variables.
   %
   Fortunately, $X_1$ is a descendant of $U$. This implies that we can learn $U$ from $X_1$ by extracting the pattern from $X_1$ which is independent of $S$.
   %
   Intuitively, this can be done through imposing $P(F(X)|S=s)=P(F(X)|S=s')$, where $F(X)$ is the invariant and fair feature representation learned for downstream prediction tasks.
    
